Training Environment for High Performance Reinforcement Learning

This paper presents Tunnel, a simple, open source, reinforcement learning training environment for high performance aircraft. It integrates the F16 3D nonlinear flight dynamics into OpenAI Gymnasium python package. The template includes primitives for boundaries, targets, adversaries and sensing capabilities that may vary depending on operational need. This offers mission planners a means to rapidly respond to evolving environments, sensor capabilities and adversaries for autonomous air combat aircraft. It offers researchers access to operationally relevant aircraft physics. Tunnel code base is accessible to anyone familiar with Gymnasium and/or those with basic python skills. This paper includes a demonstration of a week long trade study that investigated a variety of training methods, observation spaces, and threat presentations. This enables increased collaboration between researchers and mission planners which can translate to a national military advantage. As warfare becomes increasingly reliant upon automation, software agility will correlate with decision advantages. Airmen must have tools to adapt to adversaries in this context. It may take months for researchers to develop skills to customize observation, actions, tasks and training methodologies in air combat simulators. In Tunnel, this can be done in a matter of days.

==> title.tex <==
\title{A Template Training Environment for High \\Performance Aircraft Reinforcement Learning}

\begin{titlepage}

%----------------------------------------------------------------------------------------
%	TITLE SECTION
%----------------------------------------------------------------------------------------

\maketitle % Title of your document
\center % Center everything on the page

Phantom Impact Paper\\[0.4cm]

%----------------------------------------------------------------------------------------
%	LOGO SECTION
%----------------------------------------------------------------------------------------

\includegraphics[width=4cm]{images/aia.png}\\[1cm] % Include a department/university logo - this will require the graphicx package
 
%----------------------------------------------------------------------------------------
%	AUTHOR SECTION
%----------------------------------------------------------------------------------------

Author:\\
Gregory F. Search, Capt, United States Air Force\\[0.4cm]  
\begin{flushleft}
Captain Greg "Bunker" Search is an Experimental Remotely Piloted Aircraft Test Pilot with the 452nd Flight Test Squadron at Edwards AFB. He leads developmental test efforts on a variety of airborne automation efforts, including Collaborative Combat Aircraft (CCA). He holds a BS in Aeronautical Engineering and a BS in Applied Mathematics from U.S. Air Force Academy where he researched Low Cost Attritable Aircraft Technology. His focus area within his MS in Electrical Engineering from Stanford University was Signal Processing and Multimedia. As part of his MS in Flight Test Engineering at the USAF Test Pilot School, his team characterized uncertainty propagation within a laser air data system.\\[0.4cm]
\end{flushleft}

%----------------------------------------------------------------------------------------
%	ABSTRACT SECTION
%----------------------------------------------------------------------------------------
Abstract:\\
\begin{abstract}
This paper presents Tunnel, a simple, open source, reinforcement learning training environment for high performance aircraft. It integrates the F-16's 3D non-linear flight dynamics into OpenAI's Gymnasium python package. The template includes primitives for boundaries, targets, adversaries and sensing capabilities that may vary depending on operational need. This offers mission planners a means to rapidly respond to evolving environments, sensor capabilities and adversaries for autonomous air combat aircraft. It offers researchers access to operationally relevant aircraft physics. Tunnel's simple code base is accessible to anyone familiar with Gymnasium and/or those with basic python skills. This paper includes  a demonstration of a week long trade study that investigated a variety of training methods, observation spaces, and threat presentations. This enables increased collaboration between researchers and mission planners which can translate to a national military advantage. As warfare becomes increasingly reliant upon automation, software agility will correlate with decision advantages. Airmen must have tools to adapt to adversaries in this context. It may take months for researchers to develop skills to customize observation, actions, tasks and training methodologies in air combat simulators. In Tunnel, this can be done in a matter of days. 

\end{abstract} 
%----------------------------------------------------------------------------------------
%	PHANTOM SECTION
%----------------------------------------------------------------------------------------
\begin{flushleft}
\newpage   
\textbf{\emph{AI Accelerator Phantom Fellowship Program}}\\[0.4cm]
\textit{The Phantom Fellowship is a rigorous five-month career-enhancing opportunity for high-performing Department of Defense professionals to assess, develop, and gain exposure to Artificial Intelligence (AI) and Machine Learning (ML) technologies. During the program, enlisted, officer, and government civilian personnel (Phantoms) embed directly with the Department of the Air Force (DAF) \& Massachusetts Institute of Technology (MIT) AI Accelerator (AIA), a cutting-edge organization with the mission of advancing AI/ML technologies for the DOD while also addressing broader societal and ethical issues related to AI/ML.}\\[0.5cm]  
\textit{During their Fellowship, Phantoms are required to apply their newly acquired AI/ML foundational\\
knowledge to produce a short-form research paper (Impact Paper) that seeks to address an AI/ML\\
problem related to their home unit and/or career field.}\\[0.4cm]

\end{flushleft}

%----------------------------------------------------------------------------------------
%	DISCLAIMERS SECTION
%----------------------------------------------------------------------------------------

\small Disclaimers:\\
\begin{flushleft} \large
\small The views expressed in this article are those of the author(s) and do not reflect the official policy or position of the United
States Air Force, Department of Defense, or the U.S. Government.\\[0.4cm]
\small The inclusion of external links and references does not imply any endorsement by the author(s), the publishing unit, the
Department of the Air Force, the Department of Defense or any other department or agency of the U.S. Government. They are
meant to provide an additional perspective or as a supplementary resource.\\
\end{flushleft}
\end{titlepage}
